Cross-Language Question Re-Ranking

We study how to find relevant questions in community forums when the language of the new questions is different from that of the existing questions in the forum. In particular, we explore the Arabic-English language pair. We compare a kernel-based system with a feed-forward neural network in a scenario where a large parallel corpus is available for training a machine translation system, bilingual dictionaries, and cross-language word embeddings. We observe that both approaches degrade the performance of the system when working on the translated text, especially the kernel-based system, which depends heavily on a syntactic kernel. We address this issue using a cross-language tree kernel, which compares the original Arabic tree to the English trees of the related questions. We show that this kernel almost closes the performance gap with respect to the monolingual system. On the neural network side, we use the parallel corpus to train cross-language embeddings, which we then use to represent the Arabic input and the English related questions in the same space. The results also improve to close to those of the monolingual neural network. Overall, the kernel system shows a better performance compared to the neural network in all cases.

==> long-related-work-section.tex <==
%%%%%%%%%%%%%%%%%% Section 2: Related Work
\section{Related Work}
% \begin{itemize}
% \item description of the cQA task
% \item description of the cross-language cQA task
% \item cross-lingual related work (also on QA or cQA if possible)
% \item cQA related work
% \end{itemize}

% description of the cQA task \& CL cqa-task
%The full pipeline of a cQA system consists of three steps. Given a freshly asked question $q_o$, 
%\Ni retrieve a subset $Q$ of the most promising previously-asked questions in the forum;
%\Nii re-rank the questions in $Q$ on the basis of their relevance against $q_o$;
%\Niii rank the comments linked to the most relevant forum questions $q_i\in Q$ based their appropriateness to answer the new question $q_o$.
%In this work we focus on step \Nii, considering $q_o\in L$ and $Q\in L'$, where $\{L,L'\}$ are two different languages.

% \todo{Q ranking}
Question re-ranking can be approached from different fronts. \citet{Cao:2008:RQU:1367497.1367509} 
% approached it as a recommendation task: given a query question, recommend questions that could be interesting or relevant. 
tackled it by comparing representations based on topic terms graphs; i.e., by judging topic similarity and quesion's focus~\cite{duan2008searching}.
%ALL THIS WORK IS ON YAHOO ANSWERS.
% 
\citet{Jeon:2005:FSQ:1099554.1099572} and \citet{zhou2011phrase} dodged the questions' lexical gap by assessing their similarity on the basis of a (monolingual) translation model.
% ~\cite{Koehn:2003:SPT:1073445.1073462}. 
% They considered the contents of the question--answer pairs as their ``parallel'' corpus to learn the translation model from.
%ALL THIS WORK IS ON YAHOO ANSWERS.
% \citet{Jeon:2005:FSQ:1099554.1099572} had used monolingual translation as well. 
% Given a large repository of question and answer threads, they looked for highly-similar threads. The questions in the so-generated pairs compose their ``parallel'' corpus. 
\citet{wang2009syntactic} computed their similarity function on the syntactic-tree representations of the questions. %The more substructures the trees have in common, the more similar their associated questions are.
A different approach using topic modeling for question retrieval was introduced by~\citet{ji2012question} and~\citet{zhang2014question}, which use LDA topic modeling to learn the latent semantic topics %that generate question/answer pairs and use the learned topics distribution 
to retrieve similar questions.
% The recent boom in neural network approaches has also impacted question retrieval. 
\citet{dossantos-EtAl:2015:ACL-IJCNLP} applied neural networks for the same purpose. %to retrieve semantically-equivalent questions.
% ' subjects. When dealing with whole questions ---subject and (generally long) body---, they had to aggregate a bag-of-words neural network to boost the model's performance. 

% ran experiments on DBPedia on Spanish and Persian. Their models includes the following steps:
% 
%   
% 
% Interestingly, in the reported experiments their model performs around F=50, whereas the MT baseline performs around F=30. They claim that most of the MT-system errors are caused by errors in the translation of NEs.
% 
% This paper describes so called aggregated questions. Not sure if this means follow up —dialogue like— questions.
% Cross-Language Similarity Models
% CL Similarity Models applied to QA
% 
% Ture and Boschee (2016) refer to translation followed by a standard QA model as the most common approach. They use it as baseline. They also apply a manifold of features derived from word-based, 10-best, context-based, and grammar-based translations
% 1) Email from Hassan in January 8th describes them.
% 2) On meeza the files are in /data/alt/Iyas/Iyas.QCRIExperiments/datasets/semeval2016taskB/kelpFiles/datasets.shallow.trees-en-ar-en_en-REL.klp/
% 3) http://clef-qa.fbk.eu/
% 4) http://trec.nist.gov/data/qa/t2005_qadata.html
% 5) http://aclia.lti.cs.cmu.edu/ntcir8
% 6) We have already the technology to do this.
% 7) Alberto has insisted in using this kind of engine instead of Google since the generation of the SemEval datasets.
% 8) They claim that they do not translate, but they continuously do.

% \todo{cross-language related work (also on QA or cQA if possible)}
Cross-language approaches have mainly focused on QA (similar to step \Niii in the cQA pipeline). They have fostered by multiple challenges, such as 
The Multilingual QA Challenge at CLEF 2008~\cite{clef/FornerPAAFMOPRSSS08}, the NTCIR-8's Advanced Cross-lingual Information Access (ACLIA)~\cite{mitamura:10}, and the DARPA Broad Operational Language Technologies (BOLT) IR task~\cite{Soboroff:2016}. 
% consisted of retrieving short passages from Web forums.  Whereas the questions were in English, the reference texts could be in either English, Arabic, or Chinese.% 
% \footnote{The relevance of an answer is to be given by a score in range $[1,5]$ (\citet{ture-boschee:2016:EMNLP2016} mapped it to Relevant if $score>=3$; Irrelevant otherwise; which is more similar to our setting; \cf Section \abc{XX}).}  



% The Multilingual QA Challenge at CLEF 2008~\cite{clef/FornerPAAFMOPRSSS08} included both newswire and Wikipedia articles in multiple languages and focused on factoid, definitional, and closed-list questions. 
% % such as English, Spanish, German, and Basque. 
% % (similarly to the TREC 2005 QA task~\cite{Voorhees:05}). 
% The NTCIR-8's Advanced Cross-lingual Information Access (ACLIA) focused on English-\{Chinese, Japanese\} and included both factoid and complex questions~\cite{mitamura:10}. 
% % The questions were in English, whereas the target corpus consisted of newspaper articles in Japanese or Chinese.
% The %DARPA Broad Operational Language Technologies 
% BOLT IR task~\cite{Soboroff:2016} consisted of retrieving short passages from Web forums.  Whereas the questions were in English, the reference texts could be in either English, Arabic, or Chinese.% 
% \footnote{The relevance of an answer is to be given by a score in range $[1,5]$ (\citet{ture-boschee:2016:EMNLP2016} mapped it to Relevant if $score>=3$; Irrelevant otherwise; which is more similar to our setting; \cf Section \abc{XX}).}  

% \todo{MODELS: MT}
Usually the full question is translated with an out-of-the-box system to address CL-QA~\cite{Adafre:08,Hartrumpf:08,Lin:10}. 
% ~\cite{Adafre:08,Ansa:08,Dornescu:08,Hartrumpf:08,Lin:10,Sacaleanu:08,VanZaanen:08}. 
\citet{ture-boschee:2016:EMNLP2016} proposed supervised models to combine different translation settings. %: word-based, 10-best, context-based, and grammar-based. 
Some approaches translate only keywords~\cite{Ren:10,shima:10}. 
% Both questions and answers are translated using the four methods and a manifold of features is computed on the resulting versions of the pairs.
% Their baseline consists of the similarity between question and one-best translated candidate answer.
% According to this work, ``[$\ldots$] there is no prior work in the literature, where the optimal query and/or answer translation is learned via machine learning.''
% In this case, the question is given in English, whereas the answer can be in English, Arabic, or Chinese.
% \abc{%
% \todo{This could be removed or moved to 3}
% Their corpus generation approach resembles the one from SemEval's task 3 ---on which we build our evaluation framework (\cf Section~\ref{sec:taskAndCorpora}). First, candidate documents are retrieved with Indri%
% \footnote{\url{http://www.lemurproject.org/indri/}} and the relevance of the top-$k$ instances is manually annotated. 
% }
% \abc{%
% \todo{This could be removed or moved to 5}
% An interesting result of this research is that, in their MAP-based evaluation, the performance of the monolingual English model is much better than the cross-language English--Arabic model (from  $\sim 0.64$ to $\sim 0.42$). As observed in Section \abc{ref}, our models do not show such a performance degradation.
% }
%
Rather than translating, terms can be mapped across languages by means of Wordnets, Wikipedia links, or Babelnet~\cite{Bouma:08,pouranbenveyseh:2016:TextGraphs-10}.
% ~\cite{Bouma:08,Munoz:08,pouranbenveyseh:2016:TextGraphs-10}.
% As~\citet{Adafre:08}, our pre-processing is built on top of UIMA.
To the best of our knowledge, no research has been carried out on cross-language question retrieval. % for . 
% Datasets exist for English, including one on the Qatar Living forum data~\cite{nakov-EtAl:2016:SemEval2} and one on Stack Exchange~\cite{lei-EtAl:2016:N16-1}, and for Japanese~\cite{Ishikawa:10}. We build our cross-language Arabic--English dataset on top of the former one.
% In their model to approach the NTCIR-8 ACLIA challenge, \citet{shima:10} proposed an architecture consisting of four steps:
% \Ni a question analyzer determines the information need (question type, answer type, key terms, etc.) on the basis of keywords which are Google-translated from the question to the collection language;
% \Nii a retrieval strategist uses Indri, language models, and an inference network based to extract a ranked list of answer-bearing documents;
% \Niii an infomation extractor ranks candidate answers from the bearing documents \abc{check this module};
% finally, \Niv an answer generator removes duplicates and selects answers.
% 
% \todo{MODELS: (Multilingual) Semantics}
% \citet{pouranbenveyseh:2016:TextGraphs-10} 
% use the Babelfy tag and match of Google-translation with ontology types.
% designed a three-step model for cross-language QA:
% \Ni keywords extraction is performed on the basis of a MaxEnt Markov model considering $[1,\ldots,3]$-grams, POS, and IDF, among other information;
% \Nii the type of each keyword     Keyword type detection. RBF SVM classifier considering the number of words in the kw, POS, idf, etc. Additionaly, some cross-language features come into play already: Babelfy tag and match of google-translation with ontology types. The classes are 1. Type Detector, 2. Grounded Entity or 3. Neutral
%     Entity Linking & Ontology Type Extraction. Search of entities in the knowledge base by means of BabelNet and cross-language links. They search for sameAs links to English.8)
%     Answer extraction. All entities in 2-hop vicinity of the entities are pruned. At this moment the paper gets obscure. They only mention that they use the model of Camacho Collados et al. to find the most similar relation.
% 
% He runs his experiments on the QALD-5 multilingual QA dataset over DBPedia 2014, used in the QALD task at CLEF 2015: 300 training and 50 test questions in 7 languages with annotated keywords and queries. The answers have to be extracted from BDPedia. Persian is not originally included in this dataset, but the authors of this paper generated it and identified the keywords.

% In the 6th Open Challenge on Question Answering Over Linked Data rather than free text, the data is in RDF format. The dataset for the multilinguaj question answering track is a dump of DBpedia 2015 including eight languages (but not Arabic). The kind of questions are general, open-domain, and factual.

